Reflection Spectroscopy of the Black Hole Binary XTE J1752-223 in its Long-Stable Hard State

We present a detailed spectral analysis of the Black Hole Binary XTE J1752-223 in the hard state of its 2009 outburst. Regular monitoring of this source by RXTE provided high signal-to-noise spectra along the outburst rise and decay. During one full month this source stalled at $\sim$30\% of its peak count rate at a constant hardness and intensity. By combining all the data in this exceptionally-stable hard state, we obtained an aggregate PCA spectrum (3-45 keV) with 100 million counts, and a corresponding HEXTE spectrum (20-140 keV) with 5.8 million counts. Implementing a version of our reflection code with a physical model for Comptonization, we obtain tight constraints on important physical parameters for this system. In particular, the inner accretion disk is measured very close in, at $R_\mathrm{in}=1.7\pm0.4$ $R_g$. Assuming $R_\mathrm{in}=R_\mathrm{ISCO}$, we find a relatively high black hole spin ($a_*=0.92\pm0.06$). Imposing a lamppost geometry, we obtain a low inclination ($i=35\pm4$ deg), which agrees with the upper limit found in the radio ($i<49$ deg). However, we note that this model cannot be statistically distinguished from a non-lamppost model with free emissivity index, for which the inclination is markedly higher. Additionally, we find a relatively cool corona ($57-70$ keV), and large iron abundance ($3.3-3.7$ solar). We further find that properly accounting for Comptonization of the reflection emission improves the fit significantly and causes an otherwise low reflection fraction ($\sim 0.2-0.3$) to increase by an order of magnitude, in line with geometrical expectations for a lamppost corona. We compare these results with similar investigations reported for GX 339-4 in its bright hard state.

==> table.tex <==
 $                                1.06 \pm 0.07 $  & 	 $                                1.13 \pm 0.09 $  & 	 $                       1.08^{+ 0.11}_{- 0.08} $  & 	 $                       1.06^{+ 0.12}_{- 0.09} $  & 	 $                                1.04 \pm 0.10 $  & 	 $                                1.03 \pm 0.10 $  & 	 $                                0.97 \pm 0.10 $  \\
 $                                   26. \pm 6. $  & 	 $                            41.^{+ 2.}_{- 2.} $  & 	 $                                 49.0 \pm 1.9 $  & 	 $                                 54.9 \pm 1.8 $  & 	 $                         59.5^{+ 1.3}_{- 2.0} $  & 	 $                                 62.9 \pm 1.5 $  & 	 $                                 68.4 \pm 1.3 $  \\
 $                         -1.7^{+ 0.7}_{- 0.4} $  & 	 $                         -1.6^{+ 0.6}_{- 0.1} $  & 	 $                      -1.45^{+ 0.22}_{- 0.15} $  & 	 $                               -1.32 \pm 0.12 $  & 	 $                               -1.24 \pm 0.08 $  & 	 $                               -1.18 \pm 0.06 $  & 	 $                               -1.11 \pm 0.04 $  \\
 $                              1.543 \pm 0.004 $  & 	 $                              1.545 \pm 0.005 $  & 	 $                              1.545 \pm 0.005 $  & 	 $                              1.547 \pm 0.005 $  & 	 $                              1.547 \pm 0.006 $  & 	 $                              1.548 \pm 0.006 $  & 	 $                    1.549^{+ 0.010}_{- 0.004} $  \\
 $                       3.10^{+ 0.13}_{- 0.06} $  & 	 $                       3.11^{+ 0.11}_{- 0.06} $  & 	 $                       3.11^{+ 0.09}_{- 0.07} $  & 	 $                       3.09^{+ 0.12}_{- 0.06} $  & 	 $                       3.06^{+ 0.13}_{- 0.03} $  & 	 $                       3.05^{+ 0.11}_{- 0.04} $  & 	 $                                3.04 \pm 0.09 $  \\
 $                                  3.4 \pm 0.4 $  & 	 $                          3.7^{+ 0.7}_{- 0.5} $  & 	 $                          3.6^{+ 0.6}_{- 0.4} $  & 	 $                                  3.7 \pm 0.5 $  & 	 $                          3.6^{+ 0.5}_{- 0.4} $  & 	 $                                  3.6 \pm 0.4 $  & 	 $                                  3.7 \pm 0.4 $  \\
 $                         55.7^{+ 2.0}_{- 1.3} $  & 	 $                                 57.2 \pm 1.9 $  & 	 $                         57.6^{+ 2.3}_{- 1.7} $  & 	 $                            58.^{+ 3.}_{- 2.} $  & 	 $                                 58.8 \pm 2.4 $  & 	 $                                   59. \pm 2. $  & 	 $                            60.^{+ 3.}_{- 2.} $  \\
 $                                0.14 \pm 0.03 $  & 	 $                       0.16^{+ 0.03}_{- 0.02} $  & 	 $                       0.16^{+ 0.03}_{- 0.02} $  & 	 $                       0.17^{+ 0.03}_{- 0.02} $  & 	 $                       0.18^{+ 0.03}_{- 0.02} $  & 	 $                       0.18^{+ 0.03}_{- 0.02} $  & 	 $                       0.20^{+ 0.03}_{- 0.02} $  \\
 $                            0.0270 \pm 0.0002 $  & 	 $                            0.0269 \pm 0.0003 $  & 	 $                            0.0269 \pm 0.0003 $  & 	 $                            0.0269 \pm 0.0003 $  & 	 $                            0.0268 \pm 0.0003 $  & 	 $                            0.0268 \pm 0.0003 $  & 	 $                            0.0270 \pm 0.0003 $  \\
 $                            0.0011 \pm 0.0004 $  & 	 $                            0.0015 \pm 0.0003 $  & 	 $                            0.0018 \pm 0.0003 $  & 	 $                            0.0021 \pm 0.0003 $  & 	 $                            0.0024 \pm 0.0003 $  & 	 $                            0.0026 \pm 0.0003 $  & 	 $                            0.0031 \pm 0.0003 $  \\
 $                         43.3^{+ 1.3}_{- 0.6} $  & 	 $                         43.3^{+ 1.2}_{- 0.8} $  & 	 $                         43.2^{+ 1.3}_{- 0.8} $  & 	 $                         43.2^{+ 1.3}_{- 0.8} $  & 	 $                         43.2^{+ 1.1}_{- 0.7} $  & 	 $                                 43.2 \pm 0.9 $  & 	 $                                 43.2 \pm 0.8 $  \\
 $                          0.00020 \pm 0.00009 $  & 	 $                          0.00021 \pm 0.00009 $  & 	 $                          0.00019 \pm 0.00010 $  & 	 $                          0.00019 \pm 0.00010 $  & 	 $                          0.00020 \pm 0.00008 $  & 	 $                          0.00020 \pm 0.00008 $  & 	 $                          0.00021 \pm 0.00008 $  \\
 $              0.00015^{+ 0.00007}_{- 0.00005} $  & 	 $              0.00014^{+ 0.00007}_{- 0.00004} $  & 	 $                          0.00016 \pm 0.00006 $  & 	 $                          0.00016 \pm 0.00006 $  & 	 $                          0.00016 \pm 0.00006 $  & 	 $                          0.00016 \pm 0.00006 $  & 	 $              0.00017^{+ 0.00005}_{- 0.00006} $  \\
 $                              0.006 \pm 0.007 $  & 	 $                              0.006 \pm 0.007 $  & 	 $                              0.005 \pm 0.007 $  & 	 $                              0.005 \pm 0.008 $  & 	 $                    0.005^{+ 0.006}_{- 0.008} $  & 	 $                              0.005 \pm 0.007 $  & 	 $                              0.004 \pm 0.007 $  \\
 $                              0.908 \pm 0.021 $  & 	 $                              0.907 \pm 0.021 $  & 	 $                              0.904 \pm 0.022 $  & 	 $                                0.90 \pm 0.02 $  & 	 $                       0.91^{+ 0.02}_{- 0.03} $  & 	 $                              0.903 \pm 0.022 $  & 	 $                                0.90 \pm 0.02 $  \\

